A Decentralized Market Mechanism for Energy Communities under Operating Envelopes

We propose an operating envelopes (OEs) aware energy community market mechanism that dynamically charges/rewards its members based on two-part pricing. The OEs are imposed exogenously by a regulated distribution system operator (DSO) on the energy community's revenue meter and is subject to a generalized net energy metering (NEM) tariff design. By formulating the interaction of the community operator and its members as a Stackelberg game, we show that the proposed two-part pricing achieves a Nash equilibrium and maximizes the community's social welfare in a decentralized fashion while ensuring that the community's operation abides by the OEs. The market mechanism conforms with the cost-causation principle and guarantees community members a surplus level no less than their maximum surplus when they autonomously face the DSO. The dynamic and uniform community price is a monotonically decreasing function of the community's aggregate renewable generation. We also analyze the impact of exogenous parameters such as NEM rates and OEs on the value of joining the community. Lastly, through numerical studies, we showcase the community's welfare, and pricing, and compare its members' surplus to customers under the DSO's regime.

==> Notes.tex <==
Notes (after submission):
1) It is worth discussing the similarity between our non-volumetric charge and the merchandising surplus (MS) in WEM. A market mechanism is revenue-adequate if it has a non-negative profit. 
    Proposition: Our market mechanism is revenue-adequate.
The proposition is similar to the revenue adequacy result of LMP, which is then neutralized by MS, but in our case we neutralize it by the non-volumetric charge.    
